Asymptotic approximations for convection onset with Ekman pumping at low wavenumbers

Ekman pumping is a phenomenon induced by no-slip boundary conditions in rotating fluids. In the context of Rayleigh-B\'enard convection, Ekman pumping causes a significant change in the linear stability of the system compared to when it is not present (that is, stress-free). Motivated by numerical solutions to the marginal stability problem of the incompressible Navier-Stokes (iNSE) system, we seek analytical asymptotic solutions which describe the departure of the no-slip solution from the stress-free. The substitution of normal modes into a reduced asymptotic model yields a linear system for which we explore analytical solutions for various scalings of wavenumber. We find very good agreement between the analytical asymptotic solutions and the numerical solutions to the iNSE linear stability problem with no-slip boundary conditions.

==> preamble.tex <==
\textwidth 6in
\textheight 9in
\topmargin -0.5in
\oddsidemargin 0.25in

%\pagestyle{myheadings}
%\markright{Technical Note \# 0005 \copyright\ April 1996 Julien}

\catcode`\@=11      %amh allows redefinition of latex2e definitions
\newenvironment{acknowledgments}{\par\vskip 10pt plus 1pt minus 1pt}{\par}
\newcommand{\rmn}[1] {{\rm #1}}
\renewcommand{\section}{\@startsection {section}{1}{\z@}%
                                   {-1.25ex \@plus -1ex \@minus -.2ex}%
                                   {0.5ex \@plus.2ex}%
                                   {\reset@font\normalsize\bfseries}}
\renewcommand{\subsection}{\@startsection{subsection}{2}{\z@}%
                                     {-1.25ex\@plus -1ex \@minus -.2ex}%
                                     {0.5ex \@plus .2ex}%
                                     {\reset@font\normalsize\bfseries}}

\def\@biblabel#1{} % remove label from bibliography listing
\def\thebibliography#1{%
\def\bibls{\kern.065em}% for letterspacing; normally .15em
\par\vskip 1.0ex plus 1.0ex minus 0.2ex
\centerline{\hspace{1.625in}\hrulefill\hspace{1.625in}}
\nobreak
 \list{}{\labelwidth\z@ \leftmargin 2em \itemindent -2em \itemsep 1pt}
 \reset@font\small \parindent\z@
 \parskip\z@ plus .1pt\relax
 \def\newblock{\hskip .11em plus .33em minus .07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist

\catcode`\@=12      %amh @ back to normal use

\usepackage{graphics}
\usepackage{subequation}
%---------------------------------------------------------- Definitions.
\newcommand{\Rey}{\mbox{\it Re}}
\newcommand{\Pe}{\mbox{\it Pe}}
\newcommand{\Pran}{\ensuremath{\sigma}}
\newcommand{\Ra}{\mbox{\it Ra}}
\newcommand{\Ta}{\mbox{\it Ta}}
\newcommand{\Ro}{\mbox{\it Ro}}
\newcommand{\Nu}{\mbox{\it Nu}}
\newcommand{\Fr}{\mbox{\it Fr}}
\newcommand{\half}{{\textstyle{1\over 2}}}


\newcommand{\ie}{\mbox{\it i.e.}}
\newcommand{\eg}{\mbox{\it e.g.}}
\newcommand{\etc}{\mbox{\it etc.}}
\newcommand{\etal}{\mbox{\it et al.}}

\def\begineq{\begin{equation}}
\def\endeq{\end{equation}}

\def\begineqn{\begin{equation*}}
\def\endeqn{\end{equation*}}

\def\beginar{\begin{eqnarray}}
\def\endar{\end{eqnarray}}
\def\beginarn{\begin{eqnarray*}}
\def\endarn{\end{eqnarray*}}

\def\lb{\left ( }
\def\rb{\right ) }
\def\lsq{\left [ }
\def\rsq{\right ] }
\def\efma{\frac{1}{\epsilon}}
\def\efmb{\frac{\epsilon^2}}
\def\efmc{\frac{\epsilon^3}}
\def\efmd{\frac{\epsilon^4}}
\def\ema{\epsilon^{-1}}
\def\emb{\epsilon^{-2}}
\def\emc{\epsilon^{-3}}
\def\emd{\epsilon^{-4}}
\def\eme{\epsilon^{-\frac{1}{2}}}
\def\ep{\epsilon}
\def\epb{\epsilon^{2}}
\def\epc{\epsilon^{3}}
\def\eph{\epsilon^{\frac{1}{2}}}

\def\srhoz{{\overline\rho}(z)}
\def\rhoz{{\overline\rho}(Z)}
\def\drhoz{\partial_Z{\overline\rho}(Z)}
\def\sdrhoz{\partial_z{\overline\rho}(z)}
\def\src{{\cal S}}

\def\ub{{\bf u}}
\def\vb{{\bf v}}
\def\vkb{{\bf \widehat v}}
\def\dt{{\partial_T}}
\def\dx{{\partial_X}}
\def\dy{{\partial_Y}}
\def\dyy{{\partial_{YY}}}
\def\dsx{{\partial_x}}
\def\dsy{{\partial_y}}
\def\dsyy{{\partial_{yy}}}
\def\dsz{{\partial_z}}
\def\dszz{{\partial_{zz}}}
\def\dszzz{{\partial_{zzz}}}
\def\dz{{\partial_Z}}
\def\dzz{{\partial_{ZZ}}}
\def\dzzz{{\partial_{ZZZ}}}
\def\hz{{\bf\widehat z}}
\def\hy{{\bf\widehat y}}
\def\hx{{\bf\widehat x}}
\def\ldb{{\langle\hspace{-0.5em}\langle}}
\def\rdb{{\rangle\hspace{-0.5em}\rangle}}
\def\om{\mbox{\boldmath $\widehat\eta$}}
\def\omc{\mbox{\boldmath $\widehat\xi$}}
\def\zt{\mbox{\boldmath $\widehat\zeta$}}
\def\omb{\mbox{\boldmath $\omega$}}
\def\tnb{\widetilde\nabla}
\def\hnb{\widehat\nabla}
\def\tdt{{\widetilde\nabla}^2}
\def\md{D^\perp_t}

\newbox\grsign \setbox\grsign=\hbox{$>$} \newdimen\grdimen
\grdimen=\ht\grsign
\newbox\simlessbox \newbox\simgreatbox
\setbox\simgreatbox=\hbox{\raise.5ex\hbox{$>$}\llap
     {\lower.5ex\hbox{$\sim$}}}\ht1=\grdimen\dp1=0pt
\setbox\simlessbox=\hbox{\raise.5ex\hbox{$<$}\llap
     {\lower.5ex\hbox{$\sim$}}}\ht2=\grdimen\dp2=0pt
\def\simgreat{\mathrel{\copy\simgreatbox}}
\def\simless{\mathrel{\copy\simlessbox}}

\newfam\msyfam
\def\msy@{\hexnumber\msyfam}

